Expansion coefficient of the pseudo-scalar density using the gradient flow in lattice QCD

We use the Yang-Mills gradient flow to calculate the pseudo-scalar expansion coefficient $c_P^*(t_f)$. This quantity is a key ingredient to obtaining the chiral condensate and strange quark content of the nucleon using the Lattice QCD formulation, which can ultimately determine the spin independent (SI) elastic cross section of dark matter models involving WIMP-nucleon interactions. The goal, using the gradient flow, is to renormalize the chiral condensate and the strange content of the nucleon without a power divergent subtraction. Using Chiral symmetry and the small flow time expansion of the gradient flow, the scalar density at zero flow time can be related to the pseudo-scalar density at non zero flow time. By computing the flow time dependance of the pseudo-scalar density over multiple lattices box sizes, lattice spacings and pion masses, we can obtain the scalar density of the nucleon. Our lattice ensembles are $N_{f}=2+1$, PCAC-CS gauge field configurations, varying over $m_{\pi}\approx \{410,570,700\}$~MeV at $a=0.0907$~fm, with additional ensembles that vary $a\approx \{0.1095,0.0936,0.0684\} $~fm at $m_{\pi} \approx 700$~MeV.

==> FinalizedGraphs/AA0_latspace.tex <==
\begin{tabular}{lllll}
\toprule
{} &           $\chi^{2}_{pdf}$ &                          a &              b &                            c \\
\midrule
L16_Fit     &  $1.47(29) \times 10^{-4}$ &              $-1.6202(23)$ &  $0.66870(90)$ &                 $0.1307(13)$ \\
L20_Fit     &                $0.090(90)$ &              $-1.3283(16)$ &  $0.49440(59)$ &  $8.59(8.51) \times 10^{-4}$ \\
L28_Fit     &                 $0.13(12)$ &  $-9.57(1) \times 10^{-1}$ &  $0.30065(27)$ &    $-1.93(1) \times 10^{-1}$ \\
combine_Fit &                 $0.94(54)$ &                $12.6(4.4)$ &    $-6.4(2.1)$ &                  $-7.0(2.3)$ \\
\bottomrule
\end{tabular}


==> FinalizedGraphs/AA0_mpi.tex <==
\begin{tabular}{lllll}
\toprule
{} &              $\chi^{2}_{pdf}$ &                            a &              b &                           c \\
\midrule
mpi410_Fit  &                    $1.10(76)$ &                $-1.3284(16)$ &  $0.47895(56)$ &               $0.00227(98)$ \\
mpi570_Fit  &                    $1.5(1.1)$ &                $-1.3149(12)$ &  $0.48126(46)$ &  $-6.79(68) \times 10^{-3}$ \\
mpi700_Fit  &                    $0.56(52)$ &  $-1.30(0.00) \times 10^{0}$ &  $0.48489(29)$ &   $-1.61(4) \times 10^{-2}$ \\
L16_Fit     &  $2.54(2.43) \times 10^{-25}$ &                $-1.6176(27)$ &   $0.6675(11)$ &                $0.1292(14)$ \\
L20_Fit     &                   $0.085(88)$ &                $-1.3358(19)$ &  $0.49764(74)$ &               $0.00521(99)$ \\
L28_Fit     &                   $0.067(69)$ &                $-1.1743(23)$ &  $0.38712(94)$ &               $-0.0565(11)$ \\
combine_Fit &                    $0.94(54)$ &                  $12.6(4.4)$ &    $-6.4(2.1)$ &                 $-7.0(2.3)$ \\
\bottomrule
\end{tabular}

